D-Grasp: Physically Plausible Dynamic Grasp Synthesis for Hand-Object Interactions

We introduce the dynamic grasp synthesis task: given an object with a known 6D pose and a grasp reference, our goal is to generate motions that move the object to a target 6D pose. This is challenging, because it requires reasoning about the complex articulation of the human hand and the intricate physical interaction with the object. We propose a novel method that frames this problem in the reinforcement learning framework and leverages a physics simulation, both to learn and to evaluate such dynamic interactions. A hierarchical approach decomposes the task into low-level grasping and high-level motion synthesis. It can be used to generate novel hand sequences that approach, grasp, and move an object to a desired location, while retaining human-likeness. We show that our approach leads to stable grasps and generates a wide range of motions. Furthermore, even imperfect labels can be corrected by our method to generate dynamic interaction sequences.

==> sections/tables/table_exp1.tex <==
\newcommand{\greycellcol}{\cellcolor[HTML]{E4E4E4}}
\begin{table*}[t]
	\centering
	\resizebox{2\columnwidth}{!}{%
		\begin{tabular}{ll|ccc|ccc}
		
			\toprule
            & \multirow{2}{*}{Models} & \multicolumn{3}{c}{Training set} & \multicolumn{3}{c}{Test set} \\
			&  & Success [\%] $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interp. [$cm^3$] $\downarrow$ & Success [\%] $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interp. [$cm^3$] $\downarrow$  \\
			
			\midrule

			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
			& GT+PD & 0.2 & $15.8 \pm 7.9$ & 0.38 & 0.23 & 15.6 $\pm 6.6$ & 0.78 \\
% 			\rowcolor{Gray}
% 			& GraspTTA \cite{jiang2021graspTTA} & & \\
            & \greycellcol GT+IK & \greycellcol 0.25 & \greycellcol $14.8 \pm 9.1$ & \greycellcol 0.74 & \greycellcol 0.35 & \greycellcol $13.2 \pm 9.1 $ & \greycellcol 1.41\\
            
            
            & \textbf{Ours} & \textbf{0.81}  & $3.7 \pm 5.8$  & \textbf{0.10} & 0.42  & $12.4 \pm 10.4$  & \textbf{0.14}\\
            
            & \greycellcol Ours AllObj & \greycellcol 0.73 & \greycellcol $\mathbf{3.0 \pm 5.5}$ & \greycellcol - & \greycellcol \textbf{0.6} & \greycellcol $\mathbf{4.8 \pm 6.7}$ & \greycellcol -\\

			%\rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $12.6 \pm 6.5$ &  5.35 & 0.25 & $13.0 \pm 7.3 $ &  5.31 \\
			
			& \greycellcol Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & \greycellcol 0.29 & \greycellcol $14.9 \pm 10.1$ & \greycellcol 0.57 & \greycellcol 0.30 & \greycellcol $12.5 \pm 8.7 $ & \greycellcol 6.42 \\
			
			& \textbf{Ours} & 0.60 & $\mathbf{5.2 \pm 6.5}$ & \textbf{0.05} & 0.44 & 7.7 \pm 7.5 & \textbf{0.08} \\
			& \greycellcol \textbf{Ours corrected} & \greycellcol  \textbf{0.80} &  \greycellcol $\mathbf{2.2 \pm 4.6}$ & \greycellcol - & \greycellcol \textbf{0.68} & \greycellcol $\mathbf{4.0 \pm 5.8}$ & \greycellcol - \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $ 11.5 \pm 6.6$ & 2.82 & 0.28 & $11.9 \pm 8.6 $ & 2.85\\
			& \greycellcol Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & \greycellcol 0.29 & \greycellcol $13.2 \pm 9.4$ & \greycellcol 6.51 & \greycellcol 0.34 & \greycellcol $10.6 \pm 8.0 $ & \greycellcol 0.51 \\
			& \textbf{Ours} & 0.61 & 5.5 \pm 6.5 & \textbf{0.03} & 0.39 & 8.6 \pm 7.8 & \textbf{0.06} \\
			& \greycellcol \textbf{Ours corrected} & \greycellcol  \textbf{0.77} &  \greycellcol $\mathbf{2.7 \pm 5.9}$ & \greycellcol - & \greycellcol \textbf{0.66} & \greycellcol $\mathbf{5.5 \pm 7.4}$ & \greycellcol - \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}
			
			\bottomrule
			
		\end{tabular}%
	}
	% \vspace{2mm}
	\caption{\textbf{Static grasp evaluation}. 
	We compare our model with grasp samples from the DexYCB dataset (top row) or generated by a grasp synthesis method (middle and bottom row). We evaluate the baseline grasps in the simulation via PD-control (*+PD) directly or after de-noising via inverse kinematics (*+IK). \update{We observe that our method outperforms the baselines on both the training and test sets on all the metrics. The results indicate that static grasp references 1) will not lead to stable grasps when evaluated in a physics simulation and 2) suffer from interpenetration. Our method can correct the interpenetration and learn stable grasps in a dynamic setting.}
	}
	\label{tab:exp1_train}
\end{table*}{}

% \begin{table*}[]
% 	\centering
% 	\resizebox{2\columnwidth}{!}{%
% 		\begin{tabular}{lc|ccc|ccc}
		
% 			\toprule
%             & \multirow{2}{*}{Models} & \multicolumn{3}{c}{Training set} & \multicolumn{3}{c}{Testing set} \\
% 			&  & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$ & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
% 			\midrule

% 			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
% 			& GT+PD & 0.2 & $15.8 \pm 7.9$ & tbd & 0.23 & 15.6 $\pm 6.6$ & tbd \\
% % 			\rowcolor{Gray}
% % 			& GraspTTA \cite{jiang2021graspTTA} & & \\
%             & \cellcolor[HTML]{E4E4E4}GT+IK & \cellcolor[HTML]{E4E4E4}0.25 & \cellcolor[HTML]{E4E4E4}$14.8 \pm 9.1$ & \cellcolor[HTML]{E4E4E4}tbd & \cellcolor[HTML]{E4E4E4}0.35 & \cellcolor[HTML]{E4E4E4}$13.2 \pm 9.1 $ & \cellcolor[HTML]{E4E4E4}tbd\\
            
            
%             & Ours & \textbf{0.81}  & $\mathbf{3.7 \pm 5.8}$  & \textbf{0} & \textbf{0.42}  & $\mathbf{12.4 \pm 10.4}$  & \textbf{0}\\

% 			%\rowcolor{Gray}

			
% 			\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $12.6 \pm 6.5$ & tbd & 0.25 & $13.0 \pm 7.3 $ & tbd \\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $14.9 \pm 10.1$ & tbd & 0.30 & $12.5 \pm 8.7 $ & tbd \\
% 			& Ours & \textbf{0.60} & $\mathbf{5.2 \pm 6.5}$ & \textbf{0} & \textbf{0.44} & $\mathbf{7.7 \pm 7.5}$ & \textbf{0} \\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}

			
% 			\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $ 11.5 \pm 6.6$ & tbd & 0.28 & $11.9 \pm 8.6 $ & tbd\\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $ 13.2 \pm 9.4$ & tbd & 0.34 & $10.6 \pm 8.0 $ & tbd \\
% 			& Ours & \textbf{0.61} & $\mathbf{5.5 \pm 6.5}$ & \textbf{0} & \textbf{0.39} & $\mathbf{8.6 \pm 7.8}$ & \textbf{0} \\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}
			
% 			\bottomrule
			
% 		\end{tabular}%
% 	}
% 	% \vspace{2mm}
% 	\caption{Evaluation on train and test set}
% 	\label{tab:exp1_train}
% \end{table*}{}



% \begin{table}[]
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 		\begin{tabular}{lc|ccc}
		
% 			\toprule

% 			& Models & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
% 			\midrule

% 			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
% 			& GT+PD & 0.23 & 15.6 $\pm 6.6$ & tbd\\
% % 			\rowcolor{Gray}
% % 			& GraspTTA \cite{jiang2021graspTTA} & & \\
%             & GT+IK & 0.35 & $13.2 \pm 9.1 $ & tbd\\
            
%             & Ours & \textbf{0.42}  & $\mathbf{12.4 \pm 10.4}$  & \textbf{0}\\

% % 			\rowcolor{Gray}

			
% 			\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $13.0 \pm 7.3 $ & tbd \\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.30 & $12.5 \pm 8.7 $ & tbd  \\
% 			& Ours & \textbf{0.44} & $\mathbf{7.7 \pm 7.5}$ & \textbf{0}\\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}

% 					\midrule
			
% 		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $11.9 \pm 8.6 $ & tbd \\
% 			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.34 & $10.6 \pm 8.0 $ & tbd \\
% 			& Ours & \textbf{0.39} & $\mathbf{8.6 \pm 7.8}$ & \textbf{0}\\
% % 			\cmidrule(lr){2-11}
% 			% \rowcolor{Gray}
			
% 			\bottomrule
			
% 		\end{tabular}%
% 	}
% 	% \vspace{2mm}
% 	\caption{Evaluation on test set}
% 	\label{tab:exp1_test}
% \end{table}{}

==> sections/tables/table_exp1_test.tex <==
\begin{table}[]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{lc|ccc}
		
			\toprule

			& Models & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
			\midrule

			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
			& GT+PD & 0.23 & 15.6 $\pm 6.6$ & tbd\\
% 			\rowcolor{Gray}
% 			& GraspTTA \cite{jiang2021graspTTA} & & \\
            & GT+IK & 0.35 & $13.2 \pm 9.1 $ & tbd\\
            
            & Ours & \textbf{0.42}  & $\mathbf{12.4 \pm 10.4}$  & \textbf{0}\\

% 			\rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $13.0 \pm 7.3 $ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.30 & $12.5 \pm 8.7 $ & tbd  \\
			& Ours & \textbf{0.44} & $\mathbf{7.7 \pm 7.5}$ & \textbf{0}\\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}

					\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $11.9 \pm 8.6 $ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.34 & $10.6 \pm 8.0 $ & tbd \\
			& Ours & \textbf{0.39} & $\mathbf{8.6 \pm 7.8}$ & \textbf{0}\\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}
			
			\bottomrule
			
		\end{tabular}%
	}
	% \vspace{2mm}
	\caption{Evaluation on test set}
	\label{tab:exp1_test}
\end{table}{}



==> sections/tables/table_exp1_train.tex <==
\begin{table}[]
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{lc|ccc}
		
			\toprule

			& Models & Success [\%] $\uparrow$ & SimDist [mm] $\downarrow$ & Interp. [mm] $\downarrow$  \\
			
			\midrule

			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}}  
			& GT+PD & 0.2 & $15.8 \pm 7.9$ & tbd\\
			%\rowcolor{Gray}
% 			& GraspTTA \cite{jiang2021graspTTA} & & \\
            & GT+IK & 0.25 & $14.8 \pm 9.1$ & tbd\\
            
            & Ours & \textbf{0.81}  & $\mathbf{3.7 \pm 5.8}$  & \textbf{0}\\

			%\rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{DexYCB}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.25 & $12.6 \pm 6.5$ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $14.9 \pm 10.1$ & tbd \\
			& Ours & \textbf{0.60} & $\mathbf{5.2 \pm 6.5}$ & \textbf{0} \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}

			
			\midrule
			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{HO3D}}} 
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+PD & 0.28 & $ 11.5 \pm 6.6$ & tbd \\
			& Jiang \textit{et. al} \cite{jiang2021graspTTA}+IK & 0.29 & $ 13.2 \pm 9.4$ & tbd  \\
			& Ours & \textbf{0.61} & $\mathbf{5.5 \pm 6.5}$ & \textbf{0} \\
% 			\cmidrule(lr){2-11}
			% \rowcolor{Gray}
			
			\bottomrule
			
		\end{tabular}%
	}
	% \vspace{2mm}
	\caption{Evaluation on train set}
	\label{tab:exp1_train}
\end{table}{}



==> sections/tables/table_rebuttal_generalization.tex <==
\newcommand{\greycellcol}{\cellcolor[HTML]{E4E4E4}}
\begin{table}[h!]
	\centering
	\resizebox{0.78\columnwidth}{!}{%
		\begin{tabular}{l|ll|ccc}
		
			\toprule

			& & Models & Success $\uparrow$ & SimDist [mm/s] $\downarrow$ & Interp. [$cm^3$] $\downarrow$  \\
			
			\midrule
			\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{UO}}}
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{UO-1}}}
            & GT+PD & 0.41 & $10.7 \pm 9.9 $ & 0.24 \\
            & & \greycellcol \textbf{Ours} & \greycellcol \textbf{0.83}  & \greycellcol $\mathbf{3.3 \pm 7.7}$  & \greycellcol \textbf{0.0} \\

			\cmidrule{2-6}
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{UO-2}}}
            & GT+PD & 0.3 & $15.5 \pm 10.4$ & 0.49 \\
            & & \greycellcol \textbf{Ours} & \greycellcol \textbf{0.59}  & \greycellcol $\mathbf{8.4 \pm 10.4}$  & \greycellcol \textbf{0.0} \\
			
			\midrule
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{UG}}}
            & Ours PO & 0.42  & $12.4 \pm 10.4$  & 0.14 \\
%             % \rowcolor{Gray}
            & & \greycellcol \textbf{Ours AO} & \greycellcol \textbf{0.61} & \greycellcol $\mathbf{6.9 \pm 7.9}$ & \greycellcol \textbf{0.0}  \\
            % \rowcolor{Gray}

			\cmidrule{2-6}
			& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{IB}}}
            % & Flat-RL & 0.55 & 1.66 \\
%             % \rowcolor{Gray}
%             & \greycellcol Ours+static grasp & \greycellcol 0.45 & \greycellcol 1.46 \\
            & CO [11] +PD & 0.6 & $6.5 \pm 5.8$ & 11. 7 \\
%             % \rowcolor{Gray}
            & & \greycellcol \textbf{Ours} & \greycellcol \textbf{0.81}  & \greycellcol $\mathbf{1.9 \pm 3.6}$ & \greycellcol \textbf{0.19}  \\
            % \rowcolor{Gray}
			
			\bottomrule
		\end{tabular}%
	}
    \vspace{-0.2cm}
	\caption{\footnotesize{Generalization to unseen object sets (UO), a policy trained over all objects evaluated on unseen grasp labels (UG), and a policy trained and evaluated on grasp labels from HO3D images (IB).}}
	\label{tab:unseen_obj}
\end{table}{}


